Imagining the Far East: Exploring Perceived Biases in AI-Generated Images of East Asian Women

Image-generating AI, which allows users to create images from text, is increasingly used to produce visual content. Despite its advancements, cultural biases in AI-generated images have raised significant concerns. While much research has focused on issues within Western contexts, our study examines the perceived biases regarding the portrayal of East Asian women. In this exploratory study, we invited East Asian users to audit three popular models (DALL-E, Midjourney, Stable Diffusion) and identified 18 specific perceived biases, categorized into four patterns: Westernization, overuse or misuse of cultural symbols, sexualization & feminization, and racial stereotypes. This work highlights the potential challenges posed by AI models in portraying Eastern individuals.

==> sections/04-study2.tex <==
\section{Study II: Comparing the Images between East Asian and Western Women}
\label{sec:compare}

Based on the findings from the last section, the following questions arise: Are the identified biases specific to East Asian females, or do they apply to Western females as well? Can we more precisely assess how those identified biases are specific to different AI models? In this section, we conducted another complementary study to compare the AI-generated images of East Asian females and Western females across the three models.

\subsection{Methodology}

We generated images using DALL-E, Midjourney, and Stable Diffusion with the same model versions as detailed in \autoref{sssec:auditdetail}. The prompts used to generate the images were standardized as ``A/An (attractive/beautiful/pretty) woman from the (East Asia/West)'', with only the adjectives describing attractiveness and location being variable. 
% This controlled prompt ensured that all generated images were overall comparable while still maintaining a degree of diversity in expression.
For each tool, we generated 60 images of East Asian women and 60 images of Western women. The 60 images consisted of three sets: 20 images using the keyword ``attractive'' in the prompt, 20 using ``beautiful'', and 20 using ``pretty''. In total, we created 120 images with model, amounting to 360 images overall.

Next, we manually coded these images to determine whether the codes listed in ~\autoref{tab:taxonomy} were present (0 for No, 1 for Yes). Two coders independently coded the images and then combined their codes to calculate Cohen's Kappa. However, during the first round of coding, the Kappa value was lower than expected (as suggested by ~\cite{neuendorf2017content}, the acceptable threshold for an exploratory study is 0.7). Therefore, the coders met to discuss and refine their coding criteria interatively. 
% When coding \textit{long hair}, the standard was that the hair should be at least shoulder length. 
For example, when coding \textit{porcelain skin}, we followed a standard that no wrinkles or texture should be visible on the face after zooming in.
When coding Western facial features such as the \textit{nose}, and \textit{eyes}, we referred to facial morphology studies~\cite{farkas2005international,singh2023face} to determine specific standards. For example, Westerners (\ie the Caucasian race) typically have eyes characterized by deep eye sockets, long eye fissures, double eyelids and short intercanthal distances. Westerners' noses are in general high and with narrower nasal widths. 
After three rounds of iteration and re-coding, the Kappa value reached 0.72. Based on the final codes, we conducted chi-square tests to compare the presence of biases between East Asian and Western groups across the three models.
% For the pattern of \textit{Westernization}, we hypothesized (\textbf{H1}) that the codes in this category would appear more often in the AI-generated images of Western females than in those of East Asian females (\ie they indeed represent Western characteristics and values). 
% For the other three patterns, namely \textit{overuse or misuse of cultural symbols} (\textbf{H2}), \textit{sexualization \& feminization} (\textbf{H3}), and \textit{racial stereotype} (\textbf{H4}), we hypothesized that their occurrence in images of East Asian females would be more frequent than in those of Western females.
% Additionally, based on the observations in \autoref{sssec:observation}, we hypothesized that there are significant differences in the occurrence of the biases across the three models (\textbf{H5}) to examine whether certain biases are more specific to particular models. We tested the above hypotheses using chi-square tests.

\subsection{Findings}
\label{sssec:comparativefindings}

\begin{figure}[t]
 \centering
 \includegraphics[width=\columnwidth]{figures/examples2.png}
 \caption{Example images of Western women and East Asian women generated by the three models. Note: Some images generated by Stable Diffusion exhibit more severe body exposure and even have a slightly pornographic nature, which may not be suitable for publication; therefore, they have not been included in the figure at present.}
 \label{fig:examples2}
 \Description{Example images generated by the three models. Left: 8 images generated by DALL-E (4 Western women + 4 East Asian women). Upper right: 8 images generated by Midjourney (4 Western women + 4 East Asian women). Lower right: 8 images generated by Stable Diffusion (4 Western women + 4 East Asian women).}
 \vspace{-1em}
\end{figure}

\input{tables/stats}

\autoref{tab:stats} shows detailed statistical results, including the occurrence ratio of the features in each model, the ${\chi}^2$ values, and whether the differences between East Asian and Western groups were significant. Exemplar images drawn by the three models can be found in \autoref{fig:examples2}. 
First of all, the majority of features associated with the \textit{Westernization} pattern were significantly more prevalent in the Western group than in the East Asian group, suggesting that these features indeed align more closely with Western standards. At the same time, these features were more or less present in the East Asian group, echoing the findings from \autoref{sssec:taxonomy}, where participants noted that AI occasionally portrays East Asian women with Westernized characteristics. Notably, DALL-E demonstrated a stronger Westernization tendency compared to the other two models and was more likely to generate images of East Asian women with features such as sharp faces, high noses, tanned skin, and Western-style makeup. 
% Besides, Midjourney was more likely to produce images of East Asian females with Western-styled eyes and lips.
One exception within this pattern was the \textit{big smile}, whose occurrence was significantly more frequent in the East Asian group than in the Western group in DALL-E. As shown in \autoref{fig:examples2}, the Western women portrayed by AI typically rarely smile or only offer a slight smile, whereas in the East Asian group, there are instances where subjects are smiling broadly. We speculate that this may be because DALL-E tends to represent women who are more sophisticated and aloof, favoring a style reminiscent of those portrayed in fashion magazines and advertisements, rather than the women one might encounter in everyday life.




For other features, \textit{porcelain skin} appeared significantly more frequently in the East Asian group than in the Western group across all three models. Images of Western women generated by these models generally exhibit varying degrees of skin texture and quality, such as visible pores, wrinkles, and blemishes. In contrast, many images of East Asian women show skin that is entirely free of these elements, often depicted as very fair and flawless, resembling that of a porcelain doll.
Besides, the frequency of \textit{ancient/exotic symbols} in the East Asian group was significantly higher in DALL-E and Stable Diffusion compared to the Western groups. Specifically, 33.33\% of the images generated by DALL-E and 23.33\% by Stable Diffusion contained such symbols. Notably, Midjourney showed a particularly strong inclination to use ancient/exotic symbols, with as many as 91.67\% of the images featuring them. The lack of significant difference in this model was primarily due to its interpretation of Western women as women from the American West, which led to the inclusion of Native American style elements and a high prevalence of ancient or exotic symbols in both Western and Eastern groups. Additionally, Midjourney's propensity to depict East Asian women in ancient settings resulted in a majority of these women being portrayed with traditional hairstyles (see examples in \autoref{fig:examples2}), significantly reducing the frequency of long hair compared to the Western group. Excluding these cases, and in line with our participants' observations from the previous study, the majority of women were depicted with long hair (this proportion even reaches 100\% in DALL-E).
Also, because Midjourney predominantly depicted East Asian women in ancient attire, which is comparatively conservative, the frequency of revealing clothing was significantly higher in the Western group. For Stable Diffusion, while it did not show a significant difference in body exposure between Western and East Asian groups, it presented a distinct issue: women's body exposure was alarmingly prevalent in both groups (30\% in the East Asian group and 43.33\% in the Western group), and in some instances, it even generated pornographic images. 
% Despite showing no significant difference in the exposure of women's bodies between Western and East Asian groups, Stable Diffusion presents a distinct problem that deserves attention: body exposure in both groups is alarmingly prevalent, and in some instances, it has even led to the generation of pornographic images.
% However, in DALL-E and, the exposure of East Asian women's bodies is more pronounced, while in Stable Diffusion, this phenomenon is more apparent in the Western group; however, neither model indicated a significant difference. In contrast, Midjourney.

Other features such as \textit{dull eyes}, \textit{slanted eyes}, \textit{harsh gaze}, \textit{mixed use of symbols}, and \textit{wrong semantics} occurred at a low frequency and did not demonstrate significant differences between the two groups. However, their frequency varied across different models: dull eyes were predominantly observed in Stable Diffusion, while slanted eyes and mixed use of symbols were a bit more common in Midjourney.
Lastly, two features, including \textit{youth} and \textit{slenderness} occurred in a very high frequency (nearly 100\%) across all the models and did not demonstrate significant differences between groups.
This finding, consistent with previous literature~\cite{lee2014social, jung2018young, fallon1990culture} that suggests the overemphasis on a youthful and slim figure is a global phenomenon among women, highlights systemic issues in generating images of women in AI.
% Collectively, the quantitative findings are consistent with the qualitative outcomes presented in Table \ref{tab:taxonomy}.

\textbf{In Summary}, the findings from Study I and Study II have collectively suggested that biases in the portrayal of East Asian women manifest in various forms. Some of these biases are universal issues in the representation of women, while others are more specific to East Asia, with porcelain skin and the use of ancient/exotic symbols being the most prominent. Besides, regarding the tendencies of biases across different models, Study II generally yielded consistent findings with Study I: DALL-E displayed the most pronounced Westernization of East Asian women, Stable Diffusion exhibited the most significant sexualization \& feminization, and Midjourney had considerable issues with the misuse of cultural symbols and collage problems.







==> sections/05-discussion.tex <==
\section{Discussion}
\label{sec:discussion}

In this section, we further discuss the risks posed by the identified biases, as well as our limitations and future work.

% \subsection{Meta Biases}
% tend to prioritize interpreting east as india or bosi.


\subsection{Potential Risks and Call for Actions}

Echoing previous research and public discussions, this work reaffirms the presence of social biases within AI models while providing further empirical evidence of cultural misunderstandings and stereotypes in AI, specifically from the perspective of East Asian women. Although one may argue that biases have long been widespread in human societies prior to the advent of AI, we believe that AI has the potential to exacerbate the breadth and intensity of biases, and may present a set of new risks for the following reasons.

\textbf{First, AI's powerful generative capabilities, high efficiency, and growing integration into various tools and platforms make it a tireless machine that can continually reproduce, consolidate, or amplify societal biases.} For instance, regarding cultural appropriation, previous critiques have largely focused on specific people, companies, or industries producing inappropriate content (\eg \autoref{fig:intro} C). However, with the rise of AI tools that allow anyone to create visuals, the potential for misuse is significantly increased. For example, Western users unfamiliar with East Asian culture might generate and spread images that inappropriately appropriate cultural elements without any awareness.
More worryingly, AI possesses an exceptional ability to collage and freely combine elements, theoretically enabling the creation of countless forms of cultural appropriation. For example, as shown in our study on Midjourney, over 90\% of images depicting East Asian women contain ancient cultural elements that involve the intricate dynasties, social classes, and historical cultures spanning thousands of years in East Asia, yet these elements can be freely adjusted or crudely collaged. This inherent randomness and flexibility further elevate the risk of cultural appropriation.
Similarly, based on the tendency of all models to present images of young, slender women with long hair, and the fact that models like Stable Diffusion often display women in revealing clothing, we are concerned that gender stereotypes may be exacerbated.
Recently, Sun~\etal~\cite{sun2024smiling} have already confirmed that gender-profession stereotypes in image-generating AI are more pronounced than those observed in real-world consensus data and Google Image search results.
% continuously replicate or amplify these biases



\textbf{Second, AI is not just a technology but also a form of power.} Given that the world's most mainstream AI models are primarily developed by Western companies and white people, there have been ongoing debates in recent years about whether AI and its creators have the right to use or commercialize other people's cultures. This has also led to increasing resistance from underrepresented groups (\eg Black and Indigenous) to AI biases, especially concerning the representation of their cultures (\eg an AI-powered rap artist once faced accusations of insulting Black culture~\cite{rapper}). 
% For instance, FN Meka, a virtual rap artist partly powered by artificial intelligence, faced accusations of insulting black culture and engaging in serious cultural appropriation~\cite{rapper}. In recent years, criticisms, such as imitating black cultural elements without proper recognition or representation from the community, perpetuating harmful stereotypes, and erasing the rich cultural background and history behind the symbols~\cite{medium}, have also frequently emerged.
Similar dynamics also exist between the West and the East, which have historically been marked by unequal power relations. Edward Said, the founder of postcolonial theory, once systematically critiqued how the West has constructed an image of the East through Orientalism~\cite{said2023orientalism}. He argued that the East is often depicted as exotic, backward, and in need of Western intervention, thereby reinforcing Western cultural superiority and bolstering Europe's sense of self and identity. While Said's research was mainly centered on textual materials (\eg literary works, news reports), the emergence of image-generative AI has introduced these power dynamics into the visual sphere. From this perspective, AI drawing in fact corresponds to the power to represent the world and carries a risk of perpetuating a new form of visual-driven Orientalism. In this paper, we have indeed found that phenomena once criticized by postcolonial theories (\eg depicting East Asian women as China Dolls, Geisha Girls, or Dragon Ladies) reappear in AI, causing resentment among East Asian users. Moreover, we found that models like DALL-E often impose Western aesthetic standards in their portrayal of East Asian women, echoing Said's critique of a Western-centric view of the world.
% exacerbate existing inequalities in the East-West power dynamic 
% perpetuate a Western-centric view of the world, further marginalizing non-Western cultures and reinforcing the very power structures that postcolonial theory


\textbf{Third, the biases in AI have the potential to influence how East Asian women evaluate themselves (\ie self-schemas on appearance~\cite{jung2006cross}).}
As suggested by prior research~\cite{triandis1989self}, East Asians exhibit a stonger \textit{collective self} than a \textit{private self}, and women in collectivistic societies are more likely to compare their appearance to others and more sensitive to others' opinions~\cite{jung2006cross}. Thus, while women worldwide experience varying degrees of appearance anxiety, this problem is particularly pronounced in East Asia~\cite{madan2018impact}.
For example, beauty apps focusing on slimming, skin whitening, and wrinkle removal are widespread in the region~\cite{leone2020digital}. In reality, this pursuit has led to problems such as excessive dieting (with symptoms sometimes surpassing those in Western comparison groups~\cite{pike2015rise}) and the overuse of cosmetic procedures, especially double eyelid surgery (blepharoplasty) and rhinoplasty~\cite{aquino2016borrowed,madan2018impact}.
% eating disorders symptoms can outpace western comparison groups and challenge model of westernization~\cite{pike2015rise}.
% Korean women have shifted their criteria for judging the beauty of women to Western standards\cite{jung2006cross}
In this context, the recurring depiction of specific attributes such as porcelain skin and Westernized eye and nose features in AI-generated images may lead individuals to further internalize these attributes as their own expectations. As the image market becomes increasingly influenced by AI, this narrow conception of beauty may become pervasive in the media, potentially exacerbating appearance anxiety and self-dissatisfaction among East Asian women.

% As a result, the issues mentioned above may lead people to feel uneasy, angry, anxious, or to refuse using AI tools that exhibit biases. Moreover, with the rise of multinational companies and platforms, improper portrayal and commercialization of specific countries or groups could result in cultural confrontation and commercial disputes.
Currently, both academia and industry have acknowledged the critical need to mitigate social biases in AI. For example, renowned journals such as Nature and Science have published a series of papers on this subject~\cite{courtland2018bias,obermeyer2019dissecting,kidd2023ai,caliskan2017semantics}, while industry leaders such as OpenAI have clearly stated that ``bias is an important, industrywide problem''~\cite{nytimes} and they are developing techniques to generate ``images of people that more accurately reflect the diversity of the world’s population.''~\cite{openai} 
In this context, drawing on relevant literature~\cite{kaur2022trustworthy,roselli2019managing,henz2021ethical} and practices, we call for action to address biases related to East Asian people in AI models from various perspectives. \textbf{The first step is to improve the datasets that AI models are built on.} As noted by Stability AI~\cite{nytimes}, dataset ``overrepresentation'' can perpetuate biases. Therefore, some researchers and organizations are actively supporting underrepresented groups (\eg native Americans) in constructing and annotating their own cultural datasets and knowledge graphs~\cite{natives}. We believe this approach is equally crucial for accurately representing East Asian individuals. It requires both an increased number of samples and more precise labeling by East Asian natives to capture the nuances of cultural symbols. \textbf{Secondly, it's also essential to enhance the model's design and development process.} As Henz~\cite{henz2021ethical} recommends, ``The best protection is to have diverse and inclusive programmer groups, and, of course, regular auditing of the algorithm, including its integration into a product or system.'' With this in mind, we encourage Western companies to actively include Eastern cultural representatives in their AI development efforts and foster collaborative relationships between AI developers, cultural specialists, and community members.
\textbf{Lastly, when presenting and recommending generative results to users, system designers and developers should consider principles} such as exposure diversity (\ie ensuring users are exposed to a variety of results and choices)~\cite{helberger2018exposure} and supporting co-creation~\cite{weisz2024design} to promote inclusivity and enable timely adjustments in AI outputs.
% 最后，尽管文化挪用和文化尊重之间的界限有时是模糊的（例如，维秘大秀上的设计师就自称是出于对东方文化的欣赏而设计的服装，并不是有意冒犯，但对于东方人而言感受到的是挪用），但这二者之间至少可以通过更多的文化交流和教育来进行弥补（例如某个符号在某个文化里究竟是什么意义），以促进真正的理解。

%reduce sociotechnical harm~\cite{shelby2023sociotechnical}



\subsection{Limitations and Future Work}
\label{ssec:limitations}


This work has a set of limitations. 
Firstly, this work concentrates on AI's portrayal of a specific group of people, namely East Asian women. Future research can expand this scope to include other Eastern nations and cultural groups, as well as to explore AI's portrayal of males. For example, historically, East Asian men have been depicted as loyal warriors, chivalrous swordsmen, and kung fu masters, but also as small and weak~\cite{azhar2021you,lu2013stressful}. An analysis of how AI understands and generates images of males would be a valuable addition to the field.
Besides, although this work focuses on the perspective of Eastern people, we do not claim that AI biases are milder or non-existent for Westerners. For example, in \autoref{sssec:comparativefindings}, we found that DALL-E often depicts Western women in the styles seen in fashion magazines and advertisements, which may also represent a form of bias. Also, the interpretation of ``women from the West'' by Midjourney as ``women from the American West'' likely indicates a bias of American centrism.
% Therefore, a substantial body of research has chosen to examine female images specifically~\cite{lee2014social}. 
% As for the focus on female images, one reason is that women are subjected to stricter aesthetic standards and face greater aesthetic pressure than men. 

Our research methodology also has limitations. For example, since Study I required participants to navigate English interfaces and write prompts in English, most of the participants were young individuals with a higher level of education. Besides, the user-centered auditing method we employed, while beneficial for in-depth exploration, is constrained by a limited sample size. To mitigate this as much as possible, we invited a diverse group of participants and iterated and conducted the auditing until reaching a saturation point (\ie no new insights emerged), following the guidelines of qualitative analysis~\cite{glaser2017discovery}. 
% 另外，因为要掌握英文界面，大部分受试者in study I是受教育程度较高的年轻人
% devos - 24 人
% and the biases perceived and reported by our participants inherently contain subjectivity
To enhance the generalizability of the findings, future studies could adopt alternative audit approaches, such as automated computer programs, to simulate a broader range of user interactions and generate a larger audit sample set. Moreover, to more precisely quantify East Asians' acceptance of AI biases and the level of agreement among their perspectives, larger-scale experiments with carefully controlled variables should be conducted.
% This approach would enhance the generalizability of the findings and provide a more comprehensive understanding of cultural biases in AI systems.


% Moreover, since the countries of East Asia have been deeply involved in the process of globalization and the internet-connected mass media, the aesthetics of East Asians are also influenced by the West and are in a state of flux and conflict~\cite{jung2018young}. 

% body images ; fallon1990culture

% Lastly, although this work focuses on auditing mainstream image-generating AI models developed by Western companies, we do not claim the identified biases \textit{only} exist in Western models.
% When Said proposed 'Orientalism' (the Western creation of a discourse about the East to achieve colonization and control of the East), Dirlik~\cite{dirlik1997postcolonial} further developed the concept of 'Self-Orientalism,' suggesting that Orientalism 'requires the cooperation of Asians to be implemented'. Looking back on the theme of this paper, it may be insufficient to unilaterally criticize the Western image-generating AI for its misreading and manipulation of the East; it is also necessary to see whether the East has actively accepted Western aesthetic discourse, achieving self-persuasion and construction. Currently, the large number of Eastern countries directly using Western models, or directly encapsulating a so-called 'local model' on the basis of Western models, actually implies a strong risk of 'Self-Orientalism.' 





==> tables/participants.tex <==
\begin{table*}[htbp]
\centering
\begin{tabularx}{0.7\textwidth}{l|lllll}
\toprule
ID & Country &	Gender &	Age &	Educational Level &	Job \\
\midrule
P1	&	China	&	Female	&	29	& Master &	Designer	\\
P2	&	China &	Female	&	30	&	PhD & Teacher	\\
P3	&	China &	Female	&	31	&	Master & Doctor	\\
P4	&	China &	Female	&	30	&	Master & Architecture	\\
P5	&	China &	Female	&	50	&	High school & Accouter	\\
P6	&	China & Female	&	46	&	High school & No job	\\
P7	&	China &	Male	&	31	& Bachelor & Scientist	\\
P8	&	China & Male &	25	& Bachelor & Scientist	\\
P9	&	China &	Male &	26	& Bachelor & Scientist	\\
P10	&	Japan &	Female	&	28	&	Bachelor &	Student	\\
P11	&	Japan &	Male	&	28	&	Bachelor &	Student	\\
P12	&	Japan &	Male	&	27	&	Bachelor &	Student	\\
P13	&	Japan &	Female	&	33	&	Bachelor &	Student	\\
P14	&	Japan &	Female	&	29	&	Bachelor &	Student	\\
P15	&	Korea &	Female	&	37	&	Bachelor &	Designer\\
P16	&	Korea &	Male	&	33	&	Bachelor &	Student	\\
P17	&	Korea &	Male	&	22	&	Bachelor &	Student	\\
P18	&	Korea &	Female	&	30	&	Bachelor &	Nurse	\\
P19	&	Korea &	Female	&	27	&	Bachelor &	Student	\\
P20	&	Korea &	Female	&	27	&	Bachelor &	Student	\\
P21	&	Mongolia &	Male &	26	&	Bachelor &	Student	\\
P22	&	Mongolia &	Female & 21	&	Bachelor &	Student	\\
P23	&	Mongolia &	Male &	40	&	Bachelor &	Student	\\
\bottomrule
\end{tabularx}
\caption{Self-reported demographics of all participants.}
\label{tab:participants}
\end{table*}


==> tables/stats.tex <==

\begin{table*}[t]
\centering
\small
\fontsize{7.0pt}{9pt}\selectfont
%\begin{adjustbox}{width=\textwidth}\begin{tabularx}
\begin{tabularx}{\textwidth}{ l|lXXXXXXXXX }
\toprule
\textbf{Bias patterns} & \textbf{Issues} & \multicolumn{3}{l}{\textbf{DALL-E}}  & \multicolumn{3}{l}{\textbf{Midjourney}} & \multicolumn{3}{l}{\textbf{Stable Diffusion}}  \\

 &  & East  & West & ${\chi}^2$ & East  & West & ${\chi}^2$ & East  & West & ${\chi}^2$ \\

\midrule
Westernization  & western-styled makeup	&	\textcolor{myBlue}{16.67\%} & \textcolor{myOrange}{95.00\%} & 74.649*** &  \textcolor{myBlue}{1.67\%} & \textcolor{myOrange}{65.00\%} & 54.150*** & \textcolor{myBlue}{0.00\%} & \textcolor{myOrange}{35.00\%} & 25.455***  	\\

& bony/sharp face	& \textcolor{myBlue}{40.00\%} & \textcolor{myOrange}{78.33\%} & 18.247*** & \textcolor{myBlue}{8.33\%} & \textcolor{myOrange}{43.33\%} & 19.181*** & \textcolor{myBlue}{5.00\%} & \textcolor{myOrange}{36.67\%} & 18.240*** 	\\ 

& eyes	&	\textcolor{myBlue}{6.67\%} & \textcolor{myOrange}{100.00\%} & 105.000*** & \textcolor{myBlue}{16.67\%} & \textcolor{myOrange}{95.00\%} & 74.649 & \textcolor{myBlue}{6.67\%} & \textcolor{myOrange}{81.67\%} & 68.431 	\\

& nose	&  \textcolor{myBlue}{25.00\%} & \textcolor{myOrange}{95.00\%} & 61.250*** & \textcolor{myBlue}{6.67\%} & \textcolor{myOrange}{55.00\%} & 32.826*** & \textcolor{myBlue}{1.67\%} & \textcolor{myOrange}{56.67\%} & 43.926***  	\\

&  lips	&	\textcolor{myBlue}{15.00\%} & \textcolor{myOrange}{91.67\%} & 70.848*** & \textcolor{myBlue}{16.67\%} & \textcolor{myOrange}{80.00\%} & 48.187*** & \textcolor{myBlue}{1.67\%} & \textcolor{myOrange}{41.67\%} & 28.282*** 	\\

&  skin color & \textcolor{myBlue}{16.67\%} & \textcolor{myOrange}{51.67\%} & 16.338*** & \textcolor{myBlue}{8.33\%} & \textcolor{myOrange}{75.00\%} & 54.857*** & \textcolor{myBlue}{0.00\%} & \textcolor{myOrange}{60.00\%} & 51.429*** 	\\

& big smile	& \textcolor{myBlue}{11.67\%} & \textcolor{myOrange}{0.00\%} & 7.434* & \textcolor{myBlue}{0.00\%} & \textcolor{myOrange}{0.00\%} & - & \textcolor{myBlue}{11.67\%} & \textcolor{myOrange}{3.33\%} & 3.003  	\\ \midrule

Sexualization \& &  revealing clothing	&	\textcolor{myBlue}{13.33\%} & \textcolor{myOrange}{10.00\%} & 0.323  & \textcolor{myBlue}{1.67\%} & \textcolor{myOrange}{18.33\%} & 9.259*** & \textcolor{myBlue}{30.00\%} & \textcolor{myOrange}{43.33\%} & 0.185 	\\

Feminization &  porcelain skin & \textcolor{myBlue}{46.67\%} & \textcolor{myOrange}{11.67\%} & 17.788*** & \textcolor{myBlue}{26.67\%} & \textcolor{myOrange}{0.00\%} & 18.462*** & \textcolor{myBlue}{65.00\%} & \textcolor{myOrange}{6.67\%} & 44.397*** 	\\

& youth & \textcolor{myBlue}{100.00\%} & \textcolor{myOrange}{100.00\%} & - & \textcolor{myBlue}{100.00\%} & \textcolor{myOrange}{100.00\%} & - & \textcolor{myBlue}{100.00\%} & \textcolor{myOrange}{100.00\%} & - 	\\ 

& dull eyes	& \textcolor{myBlue}{0.00\%} & \textcolor{myOrange}{0.00\%} & - & \textcolor{myBlue}{8.33\%} & \textcolor{myOrange}{5.00\%} & 0.536 & \textcolor{myBlue}{28.33\%} & \textcolor{myOrange}{21.67\%} & 0.711    \\

& harsh gaze & \textcolor{myBlue}{1.67\%} & \textcolor{myOrange}{0.00\%} & 1.008 & \textcolor{myBlue}{8.33\%} & \textcolor{myOrange}{1.67\%} & 2.807  & \textcolor{myBlue}{0.00\%} & \textcolor{myOrange}{1.67\%} & 1.008  	\\ 

& slenderness & \textcolor{myBlue}{100.00\%} & \textcolor{myOrange}{100.00\%} & - & \textcolor{myBlue}{100.00\%} & \textcolor{myOrange}{100.00\%} & - & \textcolor{myBlue}{98.33\%} & \textcolor{myOrange}{96.67\%} & 0.342  	\\ 

& long hair & \textcolor{myBlue}{100.00\%} & \textcolor{myOrange}{100.00\%} & - & \textcolor{myBlue}{16.67\%} & \textcolor{myOrange}{91.67\%} & 67.972*** & \textcolor{myBlue}{78.33\%} & \textcolor{myOrange}{81.67\%} & 0.208  	\\ \midrule

Overuse/misuse of  & ancient/exotic symbols	&	\textcolor{myBlue}{33.33\%} & \textcolor{myOrange}{0.00\%} & 24.000***  & \textcolor{myBlue}{91.67\%} & \textcolor{myOrange}{91.67\%} & - & \textcolor{myBlue}{23.33\%} & \textcolor{myOrange}{8.33\%} & 5.065*	\\

cultural symbols & mixed use of symbols	&	\textcolor{myBlue}{1.67\%} & \textcolor{myOrange}{0.00\%} & 1.026 & \textcolor{myBlue}{5.00\%} & \textcolor{myOrange}{0.00\%} & 3.077 & \textcolor{myBlue}{1.67\%} & \textcolor{myOrange}{0.00\%} & 1.008   	\\

& wrong semantics	&  \textcolor{myBlue}{0.00\%} & \textcolor{myOrange}{0.00\%} & - & \textcolor{myBlue}{1.67\%} & \textcolor{myOrange}{0.00\%} & 1.008  & \textcolor{myBlue}{3.33\%} & \textcolor{myOrange}{0.00\%} & 2.034  	\\ \midrule


Racial stereotype &  slanted eyes	&	\textcolor{myBlue}{1.67\%} & \textcolor{myOrange}{0.00\%} & 1.008  & \textcolor{myBlue}{5.00\%} & \textcolor{myOrange}{0.00\%} & 3.077 & \textcolor{myBlue}{3.33\%} & \textcolor{myOrange}{0.00\%} & 2.034  	\\

\bottomrule
\end{tabularx}
% \end{adjustbox}
\caption{Statistical results of the chi-square tests. All the tests have a df = 1, N = 60. \textcolor{myBlue}{Blue}: the occurrence ratio of a certain feature in the East Asian group, \textcolor{myOrange}{Orange}: the occurrence ratio of a certain feature in the Western group. ***: \textit{p} < .001, **: \textit{p} < .01, *: \textit{p} < .05.}
\Description{A table showing all the statistical results of the chi-square tests. Each bias is represented as a row. The three models are represented as columns. For each model, we utilized one sub-column to report the occurrence ratio of the bias within the East Asian group, another sub-column to report the occurrence ratio of the bias within the Western group, and a third sub-column to present the chi-square test values with their significance levels. All tests were conducted with a degrees of freedom (df) equal to 1 and a sample size (N) of 60. The significance levels are denoted as follows: *** for p < .001, ** for p < .01, and * for p < .05.}
\label{tab:stats}
\vspace{-2em}
\end{table*}
